Network-Aware and Welfare-Maximizing Dynamic Pricing for Energy Sharing

The proliferation of behind-the-meter (BTM) distributed energy resources (DER) within the electrical distribution network presents significant supply and demand flexibilities, but also introduces operational challenges such as voltage spikes and reverse power flows. In response, this paper proposes a network-aware dynamic pricing framework tailored for energy-sharing coalitions that aggregate small, but ubiquitous, BTM DER downstream of a distribution system operator's (DSO) revenue meter that adopts a generic net energy metering (NEM) tariff. By formulating a Stackelberg game between the energy-sharing market leader and its prosumers, we show that the dynamic pricing policy induces the prosumers toward a network-safe operation and decentrally maximizes the energy-sharing social welfare. The dynamic pricing mechanism involves a combination of a locational ex-ante dynamic price and an ex-post allocation, both of which are functions of the energy sharing's BTM DER. The ex-post allocation is proportionate to the price differential between the DSO NEM price and the energy-sharing locational price. Simulation results using real DER data and the IEEE 13-bus test systems illustrate the dynamic nature of network-aware pricing at each bus, and its impact on voltage.

==> CDCComments.tex <==
Comments to author (Associate Editor)
=====================================

According to the reviewers comments and from my own reading
of the manuscript, its quality in writing and contribution
are valuable. I encourage the authors to pay attention in
details related to the concept of dynamic pricing, the
description of the employed benchmark and the discussion of
the final conclusions. Moreover, some minor typos and the
(mis)use of some words should be carefully taken into
consideration. 

---------------------
Reviewer 12 of CDC 2024 submission 1923

Comments to the author
======================

This paper introduces a pricing framework designed for
energy-sharing distribution systems where a Net Energy
Metering tariff scheme is applied at the Distribution
System Operator revenue meter. In comparison to existing
literature, this article presents innovative insights and
is well crafted.

One aspect that warrants consideration is the
appropriateness of the term "dynamic pricing" throughout
the title and body paragraphs. Notably, the manuscript
lacks an explicit explanation of time, and the problem
setting does not directly involve dynamical systems. The
mention of "dynamic pricing" in Section IV appears somewhat
abrupt. It would be beneficial to clarify whether the
pricing framework undergoes periodic calculation, perhaps
every few minutes, to account for variations in renewable
generation across different time intervals, leading to
varying energy prices at different Bus locations. This
aspect seems pivotal and warrants a remark to elucidate the
concept of dynamic pricing; otherwise, it could lead to
confusion. Several works in the literature also have
proposed dynamic pricing frameworks such as [Zeinab et. al,
TAC2023] considering the dynamics of loads like
Thermostatically Controlled Loads (TCLs). In such works,
the temporal dimension is explicitly stated.

-----------------
Reviewer 13 of CDC 2024 submission 1923

Comments to the author
======================

The contribution is quite interesting and quite aligned
with the current trends in energy systems and smart
communities.
The simplifications of the radial network to 3-phase system
(I suppose), are quite enough to illustrate the
methodology.

Nevertheless and to help the readers and the possible
public of your presentation, please consider a better
illustration for the 13-BUS power system, including the
positions of loads and renewable sources, as well as your
pi+ and pi- values. It is difficult to follow who are
dispatching power and who are consuming it, which allows to
correlate at least the behavior between the voltage and the
power demand at every bus.

-------------
Reviewer 14 of CDC 2024 submission 1923

Comments to the author
======================

The paper presents a strategy to determine dynamic pricing
policies aimed at ensuring a safe operation of distributed
generation systems. The topic is of interest in the current
context of high participation of renewable energy sources.
The paper is well-written and organized.
I only suggest the authors to correct small typos and wrong
cross-reference equations.

-----------------
CDC 2024 has access to the CrossCheck database. Read more about the
CrossCheck initiative to prevent scholarly and professional plagiarism
at http://www.crossref.org/crosscheck.html.

Submission 1923 received a cumulative similarity score 27%.

For more information about the scan, log in at
https://css.paperplaza.net with your PIN 175158 and password, enter
your CDC 2024 author workspace, and select the option 'Inspect the
reviews and decision letter' under 'Choose an option...' for submission
1923.

Similarity scores and scan reports are generated by an external
provider (iThenticate) and not by the conference.

The scan reports are stored on the iThenticate servers and not
downloaded to the conference submission system servers. Eventually the
reports are deleted from the iThenticate servers at a time determined
by conference and provider policy, after which they are no longer
available.

Please check the on-line report to understand how the similarity score
was determined and which sections of your paper may need changes.

The score and report are provided to assist you in revising your
manuscript, if necessary.

The conference will not be able to provide you a score or a report for
the revised manuscript.
